Event-Driven Testing For Edge Applications

With the rise of the Internet of Things (IoT) and Edge computing, a considerable amount of system services are moving from reliable Cloud data centers to less reliable infrastructures closer to the end-users. However, the constrained resources, unreliable communication, and varying operating conditions of IoT pose significant complexities for software vendors in testing their applications. Although several emulators exist for testing IoT systems, numerous issues can be pointed out, such as lacking support for logical dependencies and advanced fault injection capabilities, requiring manual validation of the system's behavior, or focusing on a specific platform and language. To address these limitations, we propose Frisbee: a framework for the automated testing of IoT applications. Frisbee accelerates the testing process by simplifying the spin-up of distributed virtual testbeds over Kubernetes and the description of `what-if' scenarios that integrate complex sequences of workloads and faultloads.

==> stuff.tex <==


* 1st paragraph: \textbf{Why are repeatability and reproducibility important?}. Science is a method built on an approach of gradual advance backed up by independent verification and the ability to show that your findings are correct and transparent. Academic research findings are only useful to the wider scientific community if the knowledge can be repeated and shared among research groups. As such, irreproducible and unrepeatable studies are the source of much concern within science. 

* 2nd paragraph: \textbf{What is the reproducibility crisis?} Over recent decades, science, in particular the social and life sciences, has seen increasing importance placed on the reproducibility of published studies. Large-scale efforts to assess the reproducibility of scientific publications have turned up worrying results. For example, a 2015 paper by a group of psychology researchers dubbed the “Open Science Collaboration” examined 100 experiments published in high-ranking, peer-reviewed journals. Of these 100 studies, just 68 reproductions provided statistically significant results that matched the original findings. These efforts are part of a growing field of “metascience” that aims to take on the reproducibility crisis.


